Electricity and Reserve Pricing in Chance-Constrained Electricity Markets with Asymmetric Balancing Reserve Policies

Recently, chance-constrained stochastic electricity market designs have been proposed to address the shortcomings of scenario-based stochastic market designs. In particular, the use of chance-constrained market-clearing avoids trading off in-expectation and per-scenario characteristics and yields unique energy and reserves prices. However, current formulations rely on symmetric control policies based on the aggregated system imbalance, which restricts balancing reserve providers in their energy and reserve commitments. This paper extends existing chance-constrained market-clearing formulations by leveraging node-to-node and asymmetric balancing reserve policies and deriving the resulting energy and reserve prices. The proposed node-to-node policy allows for relating the remuneration of balancing reserve providers and payment of uncertain resources using a marginal cost-based approach. Further, we introduce asymmetric balancing reserve policies into the chance-constrained electricity market design and show how this additional degree of freedom affects market outcomes.

==> Notes/DistFormulation.tex <==
In the following the base-line model \textit{chance-constrained preventive optimal power flow with symmetric reverses} (\textbf{CC-POPF-SR}) is presented.

The objective of the optimal power flow is the minimization of the total system cost, which can be calculated based on the cost functions of the substation at node $i=0$ (market), $c_0(\boldsymbol{g}^\text{p}_0)$, and distributed generators, $c_i(\boldsymbol{p}^\text{g}_i)$:

%% Generation costs: symmetric
\begin{IEEEeqnarray}{rCl}
    % c_0{\left(\boldsymbol{g}^\text{p}_0\right)} &{=}& c^\text{p}_{1,0}\left(g^\text{p}_0 {+} \alpha^\text{}_0\mathbf{\Omega}\right) {+} c^\alpha_{1,0}\alpha^\text{}_0 \IEEEyessubnumber*\label{Eq: SubstationCost}\\ 
    c_i{\left(\boldsymbol{p}^\text{g}_i\right)} &{=}& c^\text{p}_{2,i}\left(p^\text{g}_i {+} \alpha^\text{}_i\mathbf{\Omega}\right)^2 {+} c^\text{p}_{1,i}\left(p^\text{g}_i {+} \alpha^\text{}_i\mathbf{\Omega}\right) {+} c^\text{p}_{0,i}, \forall i \in \mathcal{N^+} \IEEEeqnarraynumspace \label{Eq: DGCost}
% \nomenclature[F]{$c_i\left(*\right)$}{Generation cost function \hfill} %[\SI{}\USDkWh]}
\nomenclature[V]{$p^\text{g}_i$}{Active generation at node $i$ \hfill [\SI{}\kWh]}
\nomenclature[P]{$c^\text{p}_{i,*}$}{Cost parameters of generation at node $i$ \hfill [\SI{}\USDkWhpar]}
\nomenclature[P]{$\mathbf{\Omega}$}{Sum of nodal variances, $\mathbf{\Omega} = e^T\mathbf{\omega}$ \hfill [\SI{}\kWh]}
\nomenclature[P]{\boldmath${\omega}$}{Vector of variances, $(\mbox{\boldmath$\omega$}_i\mid i= 1,...,n)$ \hfill [\SI{}\kWh]}
\nomenclature[V]{$\alpha^\text{}_i$}{Reserve participation factor of generation at node $i$ \hfill [--]}
\end{IEEEeqnarray}

Since the generated power is subject to uncertainty, it is necessary to calculate the system's expected cost for the representation of the chance-constrained model as a deterministic equivalent. The expected generation cost is given by \cite{Mieth2019}:

% Expected symmetric cost
\begin{IEEEeqnarray}{rClr}
    {\mathbb{E}} {\left[c_i{\left(\boldsymbol{p}^\text{g}_i\right)}\right]}
    &=&  c^\text{p}_i{\left(p^\text{g}_i\right)} + c^\text{p}_2\alpha_i^2s^2\hspace{-1.75\jot}, \qquad &\forall i \IEEEeqnarraynumspace
\nomenclature[P]{$s^2$}{Total sum over covariance matrix $s^2=e\Sigma e^T$ \hfill [\SI{}\kWh]}
\nomenclature[P]{$\Sigma$}{Covariance matrix of $\mbox{\boldmath$\omega, \Sigma$} = Var\left[ \mbox{\boldmath$\omega$}\right]$ \hfill [\SI{}\kWh]}
\end{IEEEeqnarray}
where $s^2$ is the total sum over the system's covariance matrix, $s^2 := e \Sigma e^T$.


The full formulation of the CC-POPF-SR is given in Model \ref{CCPOPFSRI} (\CCPOPFSRI{}).

%% CC-POPF-SR_I
\begin{model}[h!]
\caption{\CCPOPFSRI \hfill [SOCP]}
\label{CCPOPFSRI}
\begin{subequations} 
\label{Mod: CCPOPFSRI}
\begin{IEEEeqnarray}{rlll}
    \IEEEeqnarraymulticol{4}{C}{ \min~\mathbb{E}\left[\sum_{i=0}^{n} c_{i}(\boldsymbol{p}^\text{g}_i)\right]}\\ 
    \text{s.t.:} & \IEEEnonumber\\
    & (\lambda^\text{p}_0){:}\qquad & p_{0}^\text{g} - \sum_{j\in C_{0}} f_{j}^{p} = 0 \label{Eq: P substation}\\
    & (\lambda^\text{q}_0){:} & q_{0}^\text{g} - \sum_{j\in C_{i}} f_{j}^{q} = 0\\
    & (\lambda^\text{p}_i){:} & f_{i}^{p} + p_{i}^\text{g} - \sum_{j \in C_{i}} f_{j}^{p} = P_{i}^\text{D}, &\forall i \in \mathcal{N}^{+} \IEEEeqnarraynumspace\\
    & (\lambda^\text{q}_i){:} & f_{i}^{q} + q_{i}^\text{g} - \sum_{j \in C_{i}}f_{j}^{q} = Q_{i}^\text{D}, &{\forall} i \in \mathcal{N}^{+}\\
    & (\lambda^\text{p}_i){:} &  u_{i} + 2(r_{i}f_{i}^{p} + x_{i}f_{i}^{q})=u_{A_{i}},\qquad &\forall i \in \mathcal{N}^{+}\\
    & (\mu^\text{+}_i) &  u_{i}\leq u_{i}^{max}, &\forall i \in \mathcal{N}^{+}\\
    & (\mu^\text{-}_i) & -u_{i}\leq -u_{i}^{min}, &\forall i \in \mathcal{N}^{+}\\
    & (\eta^\text{}_i){:} &  (f_{i}^{p})^2+(f_{i}^{q})^2\leq(s_{i}^{max})^2, &\forall i \in \mathcal{N}^{+}\\
    & (\theta^\text{+}_i){:} &  q_{i}^\text{g}\leq \overline{Q}_{i}, &\forall g \in \mathcal{G}\\
    & (\theta^\text{-
    }_i){:} &  -q_{i}^\text{g}\leq -\underline{Q}_{i}, &\forall g \in \mathcal{G}\\
    & (\gamma^\text{}){:} &  \sum_{i=1}^{n}\alpha_{i}^{}+\alpha_{0} = 1\label{Eq: Alpha1}\\
    & (\delta^\text{+}_i){:} &  \mathbb{P}[\boldsymbol{p}_{i}^\text{g}\leq \overline{P}_{i}]\geq 1-\epsilon_{g}, &\forall i \in \mathcal{G}\label{Eq: PmaxI}\\
    & (\delta^\text{-}_i){:} &  \mathbb{P}[-\boldsymbol{p}_{i}^\text{g}\leq -\underline{P}_{i}]\geq 1-\epsilon_{g}, &\forall i \in \mathcal{G} \label{Eq: PminI}
\end{IEEEeqnarray}
\end{subequations}
\nomenclature[P]{${P_{i}^\text{D}/Q_{i}^\text{D}}$}{Active/reactive power demand at node $i$ \hfill [\SI{}\kWh]}
\nomenclature[I]{$C_{i}$}{Set of children nodes of node i \hfill}
\nomenclature[I]{$A_{i}$}{Set of ancestor nodes of node i \hfill}
\nomenclature[P]{$\epsilon_{g}$}{Probability of generation constraints violations \hfill [\%]}
\nomenclature[V]{$f^\text{p/q}_{i}$}{Active/reactive power flow along edge $i$ \hfill [p.u.]}
\nomenclature[V]{$u_{i}$}{Squared voltage magnitude at node $i$, $u_i=v_i^2$ \hfill [p.u.]}
\end{model}

The generation chance constraints \eqref{Eq: PmaxI} and \eqref{Eq: PminI} can be reformulated as second-order conic constraints \cite{Bienstock2014}, leading to modification of \CCPOPFSRI{} into Model \ref{CCPOPFSRII} (\CCPOPFSRII{}).

%% MODEL CC-PUC-SR_II
\begin{model}[h!]
\caption{\CCPOPFSRII \hfill [SOCP]}
\label{CCPOPFSRII}
\begin{subequations} 
\label{Mod: CCPOPFSRII}
\begin{IEEEeqnarray}{rlrCCCrr}
    &&\IEEEeqnarraymulticol{6}{l}{
    \min~\mathbb{E}\left[\sum_{i=0}^{n} c_{i}(p^\text{g}_i {+} \alpha^\text{}_i)\right]}
    \vspace{4\jot}
    \\
    \text{s.t.:} & & \IEEEeqnarraymulticol{5}{l}{\CCPOPFSRI{}{:} \quad} 
    & \eqref{Eq: P substation}-\eqref{Eq: Alpha1}\quad\IEEEeqnarraynumspace \label{Eq: Condensed I}\\
    & (\delta^\text{+}_i){:}
    & p_{i}^\text{g} &+& z_{\epsilon_{g}}s\alpha_i &\leq& 
    \overline{P}_{i}, \quad &\forall i \in \mathcal{G}\quad \IEEEeqnarraynumspace \label{Eq: Pmax z}\\
    & (\delta^\text{-}_i){:} \qquad
    & -p_{i}^\text{g} &+& z_{\epsilon_{g}}s\alpha_i &\leq& 
    -\underline{P}_{i}, \quad &\forall i \in \mathcal{G}\quad \IEEEeqnarraynumspace \label{Eq: Pmin z}
\end{IEEEeqnarray}
\end{subequations}
\nomenclature[P]{$z_{\epsilon_{g}}$}{Distribution's uncertainty margin associated with the probability $\left(1-\epsilon_g\right)$ \hfill [--]}
\end{model}
The parameter $z_{\epsilon_{g}}$ represents the uncertainty margin associated with the chance probability $\left(1-\epsilon_g\right)$ and the selected distribution function \cite{Roald2015}.

The price for balancing regulation, i.e., reserve provision, are given by the dual multiplier $\gamma$ of \eqref{Eq: Alpha1} \cite{Mieth2019}:
% Uniform reserve price
\begin{IEEEeqnarray}{C}
    \gamma = \frac{1}{\sum^n_{i=0} 2c_{i,2}}\left( s^2 + z_{\epsilon_g} \sum^n_{i=1} 2c_{i,2}\left(\delta^{+}_i + \delta^{-}_i \right)\right) \label{Eq: gamma}
    \nomenclature[P]{$\gamma$}{Uniform price for balancing regulation \hfill [\$]}
\end{IEEEeqnarray}

As seen in expression \eqref{Eq: gamma}, the price for balancing regulation is uniform for all of the generators providing reserves and dependent on the following factors:
\begin{itemize}
    \item Forecast uncertainty: $s$.
    \item Risk: $z_{\epsilon_g}$.
    \item Global generation costs: $2c_{i,2}$.
    \item Generation capacity limits: through the dual multipliers $\delta^{+}_i$ and $\delta^{-}_i$, respectively related to maximum and minimum generation capacity; \eqref{Eq: Pmax z}--\eqref{Eq: Pmin z}.
\end{itemize}

\subsection{Preventive OPF with SYMMETRIC reserve provision}
The main drawback of the use of $\gamma$ as reserves' price is that it is dependent on the capacity constraints of all the generators, which means that even when only a generator is operating at its rated power the system's reserve price is going to increase. Additionally, the establishment of a system-wide reserve price does not allow to prioritize the resource for their use in load balancing.


As done in \cite{Kuang2018}, it is possible to obtain the prices for reserve allocation through the optimal dual variables of the reserve participation factor $\alpha_i$ in \CCPOPFSRI{}. For this purpose, \CCPOPFSRI{} is solved and the optimal reserve participation factors are obtained:
\begin{IEEEeqnarray}{rClr}
    \alpha^{*}_i &=& \argmin{}_{\alpha_i} \text{CCPOPFSR}_\text{I}, \quad & \forall i \IEEEyessubnumber*\\
    &=& \argmin{}_{\alpha_i} \text{CCPOPFSR}_\text{II}, \quad & \forall i
\end{IEEEeqnarray}

With the obtained $\alpha^{*}_i$, a new constrain is added to \CCPOPFSRI{} where the participation factors are fixed, resulting in Model \ref{PAlphaSR} (\PAlphaSR{}).

\begin{model}[!h]
\caption{\PAlphaSR \hfill [SOCP]}
\label{PAlphaSR}
\begin{subequations} 
\label{Mod: CCPOPFSR_alpha}
\begin{IEEEeqnarray}{rllr}
    &&\IEEEeqnarraymulticol{2}{l}{
    \min~\mathbb{E}\left[\sum_{i=0}^{n} c_{i}(p^\text{g}_i {+} \alpha^\text{}_i)\right]} \vspace{4\jot}\\ 
    \text{s.t.:} & &\CCPOPFSRII{}{:} \qquad &\eqref{Mod: CCPOPFSRII}\\
    & (\gamma^\alpha_i){:} \qquad&  \alpha_{i} = \alpha^{*}_i, & \forall i \label{Eq: Price Gamma}
\end{IEEEeqnarray}
\end{subequations}
\end{model}

The application of the Karush-Kuhn-Tucker (KKT) optimality conditions on \PAlphaSR{} allows us to calculate the values of $\gamma^\alpha_i$, which set the prices for reserves allocation:
\begin{IEEEeqnarray}{r}
    \gamma^\alpha_i {=} \gamma^\alpha_0 
    + {2} {\left[\frac{\alpha_i}{c_{i,2}}{-}\frac{\alpha_0}{c_{0,2}}\right]} {s^2} 
    + {z_{\epsilon_{g}}} {s} {\left[\left(\delta_i^{+} {+} \delta_i^{-}\right) - \left(\delta_0^{+} {+} \delta_0^{-}\right)\right]},\IEEEnonumber \\
    \forall i \IEEEeqnarraynumspace
\nomenclature[V]{$\gamma^\alpha_i$}{Nodal reserve allocation price \hfill [\SI{}\USDkWh]}
\nomenclature[V]{$\gamma^\alpha$}{System-wide reserve allocation price \hfill [\SI{}\USDkWh]}
\nomenclature[V]{$\delta^{+/-}_i$}{Dual multiplier associated with capacity limits \hfill [--]}
\end{IEEEeqnarray}

Hence, the nodal prices for symmetric reserve allocation are influenced, besides the chance-constrained risk and forecast uncertainty, by:
\begin{itemize}
    \item Reserve allocation price at the slack node (substation): $\gamma^\alpha_0$.
    \item Cost-competitiveness of the provided reserve vs. that of the slack node: $\left[\frac{\alpha_i}{c_{i,2}}{-}\frac{\alpha_0}{c_{0,2}}\right]$.
    \item Nodal generation costs: $2c_{i,2}$.
    \item Own capacity limits: $\delta_i^{+} {+} \delta_i^{-}$.
    \item Slack node capacity limits: $\delta_0^{+} {+} \delta_0^{-}$.
\end{itemize}

When compared with the system-wide reserve allocation price $\gamma$, the nodal reserve price $\gamma^{\alpha}_i$ depends on the characteristic of the balancing provision at node $i$ when compared to that of the slack node. This can be particularly seen not only on the cost-competitiveness of the reserve allocation at $i$, but also on the fact that and increase in the price at the slack node results in a increase on the nodal prices. Additionally, when the slack node is limited to provide reserve due to its capacity limits ($\delta_0^{+}{>}0 \text{ or } \delta_0^{-} {>} 0$), it becomes more economically attractive to purchase reserve from the DERs due to their price reduction.

The use of nodal reserve pricing $\gamma^\alpha_i$ provides a market signal for investors as to which are the nodes that require more reserve provision, i.e., higher values of $\gamma^\alpha_i$, and are therefore produce more revenue for the provision of this service.

The nodal reserve price can be equivalently written for node $i$ based on the prices of its children nodes as:

\begin{IEEEeqnarray}{Cl}
    \gamma^\alpha_i = \frac{1}{|\mathcal{C}_i|}\sum_{j \in \mathcal{C}_i}\gamma^\alpha_j + \chi_{i,j}, \qquad &\forall i \IEEEyesnumber\IEEEyessubnumber*\\
    \IEEEeqnarraymulticol{2}{l}{\noindent{\text{where}}}\IEEEnonumber\\
    \chi_{i,j} {=} {2} {\left[\frac{\alpha_i}{c_{i,2}}{-}\frac{\alpha_j}{c_{j,2}}\right]} {s^2} 
    {+} {z_{\epsilon_{g}}} {s} {\left[\left(\delta_i^{+} {+} \delta_i^{-}\right) {-} \left(\delta_j^{+} {+} \delta_j^{-}\right)\right]}{,} &\forall {i{,}j} \IEEEeqnarraynumspace
\end{IEEEeqnarray}

Finally, the nodal reserve price can be expressed as a function of the state of the system:

\begin{IEEEeqnarray}{rCll}
    \IEEEeqnarraymulticol{3}{l}{\gamma^\alpha_i = \frac{2}{2\sum_{j=0}^n c_{2,j} -1} 
    \left[ s^2 + \psi_i + \kappa_i + \Psi \right],} &\forall i \IEEEyesnumber\IEEEyessubnumber* \label{Eq: SR Price psi}\\
    \noindent{\text{where}}\IEEEnonumber\\
    \psi_{i} &=&   \left[z_{\epsilon_g}s\left(\delta^{+}_i+\delta^{-}_i\right) - \alpha_i\frac{s^2}{c_{2,j}}\right] \sum_{j=0}^n c_{2,j}, \qquad &\forall {i} \IEEEeqnarraynumspace \\
    \kappa_i &=&  \sum_{j=0,j\neq i}^n c_{2,j}\pi^\alpha_j, & \forall {i} \IEEEeqnarraynumspace \\
    \Psi &=& z_{\epsilon_g} s \sum_{j=0}^n \left[c_{2,j}\left(\delta^{+}_j+\delta^{-}_j\right) \right] & \IEEEeqnarraynumspace
\end{IEEEeqnarray}

Equation \eqref{Eq: SR Price psi} presents a deeper insight into the factor that influence the nodal reserve prices, namely:
\begin{itemize}
    \item Forecast uncertainty and risk: $s$ and $z_{\epsilon_g}$.
    \item Nodal capacity limits, generation costs and participation factor: $\psi_i$.
    \item Prices for the rest of the system: $\kappa_i$.
    \item System-wide capacity limits: $\Psi$.
\end{itemize}

\subsection{Preventive OPF with ASYMMETRIC reserve provision}
The system's operation cost can be calculated based on the cost functions of the substation at node $i=0$ (market), $c_0(\boldsymbol{g}^\text{p}_0)$, and distributed generators, $c_i(\boldsymbol{p}^\text{g}_i)$:

%% Generation costs: asymmetric
\begin{IEEEeqnarray}{rCr}
    % c_0(\boldsymbol{g}^\text{p}_0) &{=}& c^\text{p}_{1,0}\left(g^\text{p}_0 {+} \alpha^\text{up}_0 \mathbf{\Omega}{-}\alpha^\text{dw}_0 \mathbf{\Omega}\right) \IEEEyessubnumber*\label{Eq: SubstationCost AS}\\ 
    {c_i}{(\boldsymbol{p}^\text{g}_i)} &{=}& {c^\text{p}_{2,i}} {{\left(p^\text{g}_i {+} \alpha^\text{up}_i \mathbf{\Omega}{-}\alpha^\text{dw}_i \mathbf{\Omega}\right)\hspace{-\jot}}^{2}} \hspace{-\jot}{+} c^\text{p}_{1,i} {\left(p^\text{g}_i {+} \alpha^\text{up}_i \mathbf{\Omega}{-}\alpha^\text{dw}_i \mathbf{\Omega}\right)} {+} c^\text{p}_{0,i}{,}\IEEEnonumber\\
    &&\forall i \IEEEeqnarraynumspace \label{Eq: DGCost AS}
\end{IEEEeqnarray}
 
The expected costs with asymmetric reserves provision are then given by:

% Expected asymmetric costs
\begin{IEEEeqnarray}{rClr}
    {\mathbb{E}} {\left[c_i{\left(\boldsymbol{p}^\text{g}_i\right)}\right]}
    &=&  c^\text{p}_i{\left(p^\text{g}_i\right)} + c^\text{p}_2\left(\alpha^\text{up}_i {-}\alpha^\text{dw}_i\right)^2s^2\hspace{-1.75\jot}, \qquad &\forall i \IEEEeqnarraynumspace
\end{IEEEeqnarray}

%% MODEL CC-PUC-AR
\begin{model}[h!]
\caption{\CCPOPFAR \hfill [SOCP]}
\label{CCPOPFAR}
\begin{subequations} 
\label{Mod: CCPOPFAR}
\begin{IEEEeqnarray}{rlrCCCrr}
    &&\IEEEeqnarraymulticol{6}{l}{
    \min~\mathbb{E}\left[\sum_{i=0}^{n} c_{i}(p^\text{g}_i {+} \alpha^\text{up}_i \mathbf{\Omega}{-}\alpha^\text{dw}_i\mathbf{\Omega})\right]}
    \vspace{4\jot}
    \\
    \text{s.t.:} & & \IEEEeqnarraymulticol{5}{l}{\CCPOPFSRI{}{:} \quad} 
    & \eqref{Eq: P substation}-\eqref{Eq: Alpha1}\quad\IEEEeqnarraynumspace \label{Eq: Condensed AR}\\
    & (\delta^\text{+}_i){:}
    & p_{i}^\text{g} &+& z_{\epsilon_{g}}s\alpha_i^\text{up} &\leq& 
    \overline{P}_{i}, \quad &\forall i \in \mathcal{G}\quad \IEEEeqnarraynumspace\\
    & (\delta^\text{-}_i){:} \qquad
    & -p_{i}^\text{g} &+& z_{\epsilon_{g}}s\alpha_i^\text{dw} &\leq& 
    -\underline{P}_{i}, \quad &\forall i \in \mathcal{G}\quad \IEEEeqnarraynumspace
\end{IEEEeqnarray}
\end{subequations}
\nomenclature[V]{$\alpha_i^\text{up}$}{Nodal participation factor for balancing demand increase \hfill [--]}
\nomenclature[V]{$\alpha_i^\text{dw}$}{Nodal participation factor for balancing demand decrease \hfill [--]}
\end{model}

The application of the KKT optimality conditions on an extended \CCPOPFAR{} with the optimal values of $\alpha_i^\text{dw} \text{ and } \alpha_i^\text{dw}$ fixed, allows us to calculate the values of $\gamma^{\alpha,\text{up}}_i$ and $\gamma^{\alpha,\text{dw}}_i$, which set the prices for reserves allocation:

\begin{IEEEeqnarray}{rCr}
    \gamma_i^{\alpha,\text{up}} &\hspace{-\jot} {=}& \gamma_0^{\alpha,\text{up}} 
    \hspace{-\jot} {+} {2} {\left[\frac{\left(\alpha^\text{up}_i {-}\alpha^\text{dw}_i\right)}{c_{i,2}} {-} \frac{\left(\alpha^\text{up}_0 {-}\alpha^\text{dw}_0\right)}{c_{0,2}}\right]} {s^2}\hspace{-\jot}  
    {+} z_{\epsilon_{g}}s{\left[\delta_i^{+} {-} \delta_0^{+}\right]}{,} \IEEEnonumber \\ &&\forall i \IEEEyessubnumber*\IEEEeqnarraynumspace\\
    \gamma_i^{\alpha,\text{dw}} &\hspace{-\jot} {=}& \gamma_0^{\alpha,\text{dw}} 
    \hspace{-\jot} {+} {2} {\left[\frac{\left(\alpha^\text{dw}_i {-}\alpha^\text{up}_i\right)}{c_{i,2}} {-} \frac{\left(\alpha^\text{dw}_0 {-}\alpha^\text{up}_0\right)}{c_{0,2}}\right]} {s^2} \hspace{-\jot} {+}  z_{\epsilon_{g}}s{\left[\delta_i^{-} \hspace{-\jot} {-} \delta_0^{-}\right]}{,} \IEEEnonumber \\ &&\forall i \IEEEeqnarraynumspace
\end{IEEEeqnarray}

\section{Corrective OPF}

==> Notes/InsufficientWind.tex <==
\section{OPF with Asymmetric Reserves - Insufficient RES}

The system's operation cost can be calculated based on the scheduling with insufficient RES, i.e, when downward imbalances must be covered; which is given by:

%% Generation costs: asymmetric
\begin{IEEEeqnarray}{rCr}
    {c^\text{-}_i}{(\boldsymbol{p}_{i})} &{=}& {c^\text{p}_{2,i}} {{\left(p_{i} {+} \alpha^{-}_i \mathbf{\Omega^{-}}\right)\hspace{-\jot}}^{2}} \hspace{-\jot}{+} c^\text{p}_{1,i} {\left(p_{i} {+} \alpha^{-}_i \mathbf{\Omega^{-}}\right)} {+} c^\text{p}_{0,i}, \quad
    \forall i. \IEEEeqnarraynumspace \label{Eq: GCost AS}
\end{IEEEeqnarray}
 
The expected costs with asymmetric reserves provision are then given by (see Appendix \ref{App: Asymmetric cost - Insufficient} for detailed derivation):

% Expected asymmetric costs
\begin{IEEEeqnarray}{r}
    {\mathbb{E}} {\left[c_i^\text{-}{\left(\boldsymbol{p}_{i}\right)}\right]}
    {=}  c^\text{p}_i{\left(p_{i}\right)}
    {+}  \mu^\pm {\left(
    2 c^\text{p}_{2,i} p_i  
    {+} c^\text{p}_{1,i}
    \right)}\alpha^{-}_i {+} c^\text{p}_{2,i} \left(s \alpha^{-}_i \right)^2 \hspace{-1\jot}{,}
    \forall i. \IEEEeqnarraynumspace
\end{IEEEeqnarray}

The optimal power flow with asymmetric balancing and insufficient wind is presented in Model \ref{CCPOPFABIW} (\CCPOPFABIW).
%% MODEL CC-PUC-AR
\begin{model}[h!]
\caption{\CCPOPFABIW \hfill [QP]}
\label{CCPOPFABIW}
\begin{subequations} 
\label{Mod: CCPOPFAB}
\begin{IEEEeqnarray}{rrlr}
    &\IEEEeqnarraymulticol{3}{l}{
    \minimize~
    c^\text{p}_i{\left(p_{i}\right)} 
    {+} c^\text{p}_i{\left(p_{i}\right)}
    {+}  \mu^\pm {\left(
    2 c^\text{p}_{2,i} p_i  
    {+} c^\text{p}_{1,i}
    \right)}\alpha^{-}_i {+} c^\text{p}_{2,i} \left(s \alpha^{-}_i \right)^2
    }
    \vspace{4\jot}
    \\
    \text{s.t.} & & \IEEEeqnarraymulticol{1}{l}{\CCPOPFSBI{}{:} \quad} 
    & \eqref{Eq: P Balance}{-}\eqref{Eq: Fmax}\IEEEeqnarraynumspace \label{Eq: Condensed AB}\\
    & (\chi^\text{+/-}_u){:}  \quad &\sum_{i=1}^{n}\alpha_{i,u}^\text{+/-} = 1, & \forall u \IEEEeqnarraynumspace\\
    & (\gamma^\text{+/-}){:} \quad &  \sum_{i=1}^{n}\alpha_{i}^\text{+/-} = 1, &\forall i \IEEEeqnarraynumspace\\
    & (\kappa^\text{+/-}_i){:} \quad &  \alpha_i\boldsymbol{\Omega^\text{+/-}} = \sum_u \left(\alpha^\text{+/-}_{i,u}\boldsymbol{\omega}^\text{+/-}_u\right), & \forall i \IEEEeqnarraynumspace\\ 
    & (\delta^{+}_i){:} \quad 
    & p_{i} + z_{\epsilon_{g}}s^\pm\alpha_i^{-} \leq 
    \overline{P}_{i}, &\forall i \IEEEeqnarraynumspace\\
    & (\delta^{-}_i){:} \quad 
    & -p_{i} + z_{\epsilon_{g}}s^\pm\alpha_i^{+} \leq 
    -\underline{P}_{i}, \quad &\forall i \IEEEeqnarraynumspace
    \vspace{-4\jot}
\end{IEEEeqnarray}
\end{subequations}
\nomenclature[V]{$\alpha_i,\alpha_i^\text{+/-}$}{Net and directional participation factors for system-wide imbalances \hfill [--]}
\end{model}


\subsection{Nodal balancing prices}
The generator $i$ profit-maximization problem based on nodal participation factors can be written as:
\begin{IEEEeqnarray}{rlrCl}
    \maximize &  
    \IEEEeqnarraymulticol{3}{l}{ \quad \pi_{i}^\text{p} p_{i} + {\pi^{+}_{i}  \alpha_{i}^{+} } + {\pi^{-}_{i}  \alpha_{i}^{-} } - {c_{i}}{\left(p_{i}\right)} } \IEEEnonumber\\
    &&\IEEEeqnarraymulticol{3}{r}{- 
    \mu^\pm {\left(
    2 c^\text{p}_{2,i} p_i  
    {+} c^\text{p}_{1,i}
    \right)}\alpha^{-}_i 
    {+} c^\text{p}_{2,i}\left(\alpha^{-}_i s\right)^2
    } 
    \IEEEyesnumber\label{Eq: Profit max AR}\IEEEyessubnumber*\\
    \text {s.t.} \IEEEnonumber\\
    &\left( \delta_{i}^{+}\right): \quad & p_{i} + z_{\epsilon_{g}}s^\pm\alpha_i^{-} &\le& \overline{P}_i \\
    &\left(\delta_{i}^{-} \right):& -p_{i} + z_{\epsilon_{g}}s^\pm\alpha_i^{+} &\le& \underline{P}_i 
\end{IEEEeqnarray}

As in Section \ref{Sec: Symmetric OPF}, the values of $\gamma^\text{+/-}$ and $\kappa^\text{+/-}_i$ are unique. Therefore, the upward and downward balancing prices are equal for the whole system, and given by (see derivation on Appendix \ref{App: Asymmetric price}:
\begin{IEEEeqnarray}{rCl}
    \pi^{+} &{=}& \frac{1}{|\mathcal{G}|} \sum_{i}\left[ z_{\epsilon_g}s^\pm \delta_{i}^{-}\right], \IEEEeqnarraynumspace\IEEEyesnumber\IEEEyessubnumber*\label{Eq: pi_alpha up}\\
    \pi^{-} &{=}& \frac{1}{|\mathcal{G}|} \sum_{i}\left[\mu^\pm {\left(
    2 c^\text{p}_{2,i} p_i  
    {+} c^\text{p}_{1,i}
    \right)} 
    {+} c^\text{p}_{2,i}\alpha^{-}_is^2 + z_{\epsilon_g}s^\pm \delta_{i}^{+}\right]. \IEEEeqnarraynumspace\label{Eq: pi_alpha dw}
\end{IEEEeqnarray}

\subsection{Node-to-node balancing prices}
The generator $i$ profit-maximization problem based on nodal participation factors can be written as:
\begin{IEEEeqnarray}{rlrCl}
    \maximize &  
    \IEEEeqnarraymulticol{4}{l}{ \quad \pi_{i}^\text{p} p_{i} {+} {\sum_{u}\left(\pi^{+}_{i,u}  \alpha_{i,u}^{+} + \pi^{-}_{i,u}  \alpha_{i,u}^{-} \right)} {-} {c_{i}}{\left(p_{i}\right)} {-} c^{-}_{i,u}}  \IEEEyesnumber\label{Eq: Profit max Nodal AR} 
    \IEEEyessubnumber*\IEEEeqnarraynumspace\\
    \text {s.t.} \IEEEnonumber\\
    &\left( \delta_{i}^{+}\right): \quad& p_i  + z s^\pm \left(\frac { \sum_u \left( \alpha_{i,u}^{-}\omega_{u}^{-} \right)}{\Omega^{-}}\right) &\le& \overline{P}_i \\
    &\left(\delta_{i}^{-} \right):& -p_i + z s^\pm \left(\frac { \sum_u \left( \alpha_{i,u}^{+}\omega_{u}^{+} \right)}{\Omega^{+}}\right) &\le& \underline{P}_i \\
    \text{where} \IEEEnonumber\\
    \IEEEeqnarraymulticol{4}{l}{c^{-}_{i,u} =  
    \mu^\pm {\left(
    2 c^\text{p}_{2,i} p_i  
    {+} c^\text{p}_{1,i}
    \right)} {\smashoperator{\sum_{u}} {\left(\frac  {\alpha_{i,u}^{-} \omega_{u}^{-}}{\Omega^{-}} \right)}}} \IEEEnonumber\\
    &&\IEEEeqnarraymulticol{3}{r}{\hspace{2\jot} {+} c^\text{p}_{2,i}\left({\smashoperator{\sum_{u}} {\left(\frac  {\alpha_{i,u}^{-} \omega_{u}^{-}}{\Omega^{-}} \right)}}s\right)^2.} \IEEEeqnarraynumspace
\end{IEEEeqnarray}

Based on the KKT for \eqref{Eq: Profit max Nodal AR}, the balancing prices $\pi^{+}_{i,u}$ and $\pi^{-}_{i,u}$ for generator $i$ are given by:
\begin{IEEEeqnarray}{ll}
    \pi^{+}_{i,u} {=} \beta_u^{+} 
    z_{\epsilon_g} s^\pm {\delta_{i}^{-}}
    {,} \qquad &\forall i,k \IEEEeqnarraynumspace \label{Eq: Pi gamma_ij def up} \IEEEyesnumber\IEEEyessubnumber*\\
    \pi^{-}_{i,u} {=} \beta_u^{-} {\left[
    \mu^\pm {\left(
    2 c^\text{p}_{2,i} p_i  
    {+} c^\text{p}_{1,i}
    \right)}
    {+} 2c^\text{p}_{2,i} s^2 \alpha^{-}_i
    {+} {z_{\epsilon_g}} s^\pm {\delta_{i}^{+}}
    \right]},
    &{\forall i,k.} \IEEEeqnarraynumspace
     \label{Eq: Pi gamma_ij def dw}
\end{IEEEeqnarray}

As with the system's node-to-node balancing price, the directional node-to-node prices do not depend of the generator node $i$ providing the balancing services, which leads to
\begin{IEEEeqnarray}{rCll}
    \pi^\text{+/-}_{u} &=& \beta_u^\text{+/-} \pi^\text{+/-}
    {,} \qquad &\forall u. \IEEEeqnarraynumspace
\end{IEEEeqnarray}


\newpage

\subsection{Asymmetric Expected Cost Derivation - Insufficient Wind}\label{App: Asymmetric cost - Insufficient}

In the case of insufficient wind, generator $i$'s cost can be expressed in terms of the negative imbalance by
\begin{IEEEeqnarray}{rCll}
    {c^\text{-}_i}{(\boldsymbol{p}_{i})} &{=}& {c^\text{p}_{2,i}} {{\left(p_{i} {+} \alpha^{-}_i \mathbf{\Omega^{-}}\right)\hspace{-\jot}}^{2}} \hspace{-\jot}{+} c^\text{p}_{1,i} {\left(p_{i} {+} \alpha^{-}_i \mathbf{\Omega^{-}}\right)} {+} c^\text{p}_{0,i}, \quad
    \forall i. \IEEEeqnarraynumspace
\end{IEEEeqnarray}

The expected value of $c^\text{-}_i$ can be calculated as:
\begin{IEEEeqnarray}{rCll}
    \Expected{c^\text{-}_i{(\boldsymbol{p}_{i})}} & {=} & \Expected{{c^\text{p}_{2,i}} {{\left(p_{i} {+} \alpha^{-}_i \mathbf{\Omega^{-}}\right)\hspace{-\jot}}^{2}} \hspace{-\jot}{+} c^\text{p}_{1,i} {\left(p_{i} {+} \alpha^{-}_i \mathbf{\Omega^{-}}\right)} {+} c^\text{p}_{0,i}}{,}
    \IEEEnonumber \\
    &&& \hspace{-8\jot} \forall i \IEEEeqnarraynumspace \\
    & {=} &
    c_i\left( p_{i} \right) + \Expected{Z_i}, & \hspace{-8\jot} \forall i \IEEEeqnarraynumspace \IEEEyessubnumber
\end{IEEEeqnarray}
\vspace{-2\jot}
where
\vspace{-2\jot}

\begin{IEEEeqnarray}{rCll}
    Z_i & = & 2 c^\text{p}_{2,i} p_i \alpha^{-}_i\Omega^{-} {+} c^\text{p}_{2,i} \left( \alpha^{-}_i\Omega^{-} \right)^2 + c^\text{p}_{1,i} \alpha^{-}_i\Omega^{-},
    & \quad \forall i. \IEEEyessubnumber*\IEEEeqnarraynumspace \label{Eq: Z_i}
\end{IEEEeqnarray}

\noindent Factorizing we can separate $Z_i$ into $Z_i^a$, and $Z_i^b$
\begin{IEEEeqnarray}{rCll}
    \Expected{Z_i} & {=} & \Expected{Z_i^a} + \Expected{Z_i^b}, &\forall i \\
    Z_i^a & {=} & \left( 2 c^\text{p}_{2,i} p_i + c^\text{p}_{1,i}\right) \alpha^{-}_i\Omega^{-}, &\forall i\IEEEyessubnumber*\\
    Z_i^b & {=} & c^\text{p}_{2,i}\left( \alpha^{-}_i\Omega^{-} \right)^2, &\forall i\\
    %
    \noalign{\noindent using \eqref{Eq: Expected up dw} and \eqref{Eq: Expected square up dw}, we obtain
    \vspace{2\jot}}
    \Expected{Z_i^a} & {=} & \mu^\pm \left( 2 c^\text{p}_{2,i} p_i + c^\text{p}_{1,i}\right) \alpha^{-}_i, &\forall i\\
    \Expected{Z_i^b} & {=} & c^\text{p}_{2,i} s^2 \left( \alpha^{-}_i \right)^2, &\forall i\\
    %
    \noalign{\noindent thus,
    \vspace{2\jot}}
    \Expected{Z_i} & {=} & \mu^\pm \left( 2 c^\text{p}_{2,i} p_i {+} c^\text{p}_{1,i}\right) \alpha^{-}_i {+} c^\text{p}_{2,i} s^2 \left( \alpha^{-}_i \right)^2,  \quad &\forall i.\\
    \noalign{\noindent Finally, we obtain that the expected cost is given by
    \vspace{2\jot}}
    \IEEEeqnarraymulticol{4}{l}{\Expected{c^\text{-}_i{(\boldsymbol{p}_{i})}} {=} c^\text{p}_i{\left(p_{i}\right)}
    +  \mu^\pm {\left(
    2 c^\text{p}_{2,i} p_i  
    {+} c^\text{p}_{1,i}
    \right)}\alpha^{-}_i + c^\text{p}_{2,i} s^2 \left( \alpha^{-}_i \right)^2} \IEEEnonumber\\
    &&& , \forall i. \IEEEeqnarraynumspace
\end{IEEEeqnarray}

\subsection{Asymmetric Price Derivation - Insufficient}\label{App: Asymmetric price - insufficient}
KKT for Model \ref{CCPOPFAB}:
\begin{IEEEeqnarray}{rlr}
    \left(p_{i}\right){:} \quad & \IEEEeqnarraymulticol{2}{l}{\lambda_{i} {+} 2 c_{2,i} \left[p_{i} {+} \mu^\pm \alpha^{-}_i\right] {+} c_{1,i} {+} \delta_{i}^{+} {-} \delta_{i}^{-}=0, } \IEEEnonumber\\
    && \forall i \IEEEyesnumber\IEEEyessubnumber*\IEEEeqnarraynumspace\\
    \left(f_{i,j}\right){:}\quad& -\lambda_{i} +\psi_{i,j}+\eta_{i,j}^{+}-\eta_{i,j}^{-}=0, &\forall \{i,j\} \in \mathcal{L}\IEEEeqnarraynumspace\\
    \left(\alpha_{i,u}^{+}\right){:}\quad &\chi^{+}_{u}-\kappa^{+}_{i} \omega^{+}_{u}=0, &\forall i, k\IEEEeqnarraynumspace \\
    \left(\alpha_{i,u}^{-}\right){:}\quad &\chi^{-}_{u}-\kappa^{-}_{i} \omega^{-}_{u}=0, &\forall i, k\IEEEeqnarraynumspace\\
    \left(\alpha_{i}^{+}\right){:}\quad & 
    \IEEEeqnarraymulticol{2}{l}{\mu^\pm {\left(
    2 c^\text{p}_{2,i} p_i  
    {+} c^\text{p}_{1,i}
    \right)}
    {+} 2c^\text{p}_{2,i} s^2 \alpha^{+}_i } \IEEEnonumber\\
    \IEEEeqnarraymulticol{3}{r}{{-} \gamma^{+} {+} \kappa^{+}_{i} \Omega^{+} {+} z_{\epsilon_g}  {s^\pm} \delta_{i}^{-} {=} 0 {,} \forall i} \IEEEeqnarraynumspace\label{Eq: KKT alpha_i up}\\
    \left(\alpha_{i}^{-}\right){:}\quad & 
     -\gamma^{-} {+} \kappa^{-}_{i} \Omega^{-} {+} z_{\epsilon_g}  {s^\pm} \delta_{i}^{+} {=} 0 {,} \IEEEnonumber\\
    &&\forall i \IEEEeqnarraynumspace\label{Eq: KKT alpha_i dw}\\
    \left(\theta_{i}\right){:}\quad& \frac{-1}{X_{i j}}\left[\psi_{i j}-\psi_{j i}\right]=0, &\forall i.\IEEEeqnarraynumspace
\end{IEEEeqnarray}


==> Notes/SC_OPF.tex <==
\section{Security Constrained OPF}
The wholesale security-constrained market can modelled based on the base (precontingency) state $k{=}0$ and contingency states $k \in \{1,..., \mathcal{K}\}$. 

\subsection{Contingencies}
Contingencies can be of different nature:

\subsubsection{Controllable generators} the generated power and balancing participation will vary for each contingency state and be limited by the binary parameter $\tau^{g,k}_{i}$, which indicates whether the generator $i$ is active during contingency $k$.
\begin{IEEEeqnarray}{rCll}
    \tau^{g,k}_{i}\underline{P}_{i} \leq \boldsymbol{p}_{i}^k &\leq& \tau^{g,k}_{i}\overline{P}_{i}, \quad &\forall i, k \IEEEyesnumber\IEEEyessubnumber*\\
    \alpha_i^k &\leq& \tau^{g,k}_{i}, &\forall i, k.\\
    \noalign{\noindent In the corrective security-constrained OPF, there is the possibility for generators to used upward or downward reserves, respectively $r^\text{up}_{i}$ and $r^\text{dw}_{i}$, to respond to contingencies:
    \vspace{2\jot}}
    -r^\text{up}_{i} \leq p_{i}^k - p_{i}^{k=0} &\leq& r^\text{up}_{i}, &\forall i, k.
\end{IEEEeqnarray}

\subsubsection{Uncontrollable generators} the disconnection of an uncontrollable RES generator $u$ during contingency $k$ can be modelled by its forecasted output and the binary parameter $\widetilde{\tau}^{k}_{u}$.
\begin{IEEEeqnarray}{rCll}
    \boldsymbol{\widetilde{p}}_u^k &=& \widetilde{P}_u^k + \boldsymbol{\omega}_u^k, \quad &\forall u, k \IEEEyesnumber\IEEEyessubnumber*\\
    \noalign{\noindent where
    \vspace{2\jot}}
    \widetilde{P}_u^k &=& \widetilde{\tau}^{k}_{u}\widetilde{P}_u^{k=0}, &\forall u, k\\
    \boldsymbol{\omega}_u^k &=& \widetilde{\tau}^{k}_{u}\boldsymbol{\omega}_u^{k=0}, &\forall u, k.\\
    \noalign{\noindent The total system imbalance and its properties are then calculated for each contingency
    \vspace{2\jot}}
    \Omega^k &=& \sum_u{\boldsymbol{\omega}^k_u}, \qquad & \IEEEeqnarraynumspace \\
    \alpha^k_i\Omega^k &=& \sum_u\left(\alpha^k_{i,u}\boldsymbol{\omega}^k_u\right), \qquad &\forall i. \IEEEeqnarraynumspace
\end{IEEEeqnarray}

\subsubsection{Lines} line $\{i,j\}$'s disconnection is modelled with the binary parameter $\tau^{l,k}_{i,j}$:
\begin{IEEEeqnarray}{rCll}
    -\tau^{l,k}_{i,j}\overline{F}_{i} \leq f_{i,j}^k &\leq& \tau^{l,k}_{i,j}\overline{F}_{i,j}, \quad &\forall i,j \in \mathcal{C}_i, k \IEEEyesnumber
\end{IEEEeqnarray}

\begin{comment}
The expected cost \eqref{Eq: Objective SC SB} is given by:
\begin{IEEEeqnarray}{C}
    c_i{\left(\boldsymbol{p}^\text{}_i\right)} {=} c^\text{p}_{2,i}\boldsymbol{p}_i^2 
    {+} c^\text{p}_{1,i}\boldsymbol{p}^\text{}_i
    {+} c^\text{p}_{0,i}, \qquad \forall i. \IEEEeqnarraynumspace \label{Eq: GCost SC}
\end{IEEEeqnarray}
\end{comment}

The full security-constrained OPF with symmetric balancing (\SCOPFSBI) and chance-constrained generation is presented in Model \ref{SCOPFSBI}.


\begin{model}[h!]
\caption{\SCOPFSBI \hfill [QP]}
\label{SCOPFSBI}
\begin{subequations} 
\label{Mod: SCOPFSBI}
\begin{IEEEeqnarray}{rlll}
    \IEEEeqnarraymulticol{4}{C}{ \minimize~\sum_{i=0}^{n} \left(\Expected{c_{i}(\boldsymbol{p}^\text{}_i)} + c^\text{up}_i r^\text{up}_i  + c^\text{dw}_i r^\text{dw}_i\right)} \label{Eq: Objective SC SB}\\ 
    \text{s.t.:} & \IEEEnonumber\\
    & (\lambda^k_i){:} \quad & p_{i}^k + \widetilde{P}_i^k - D_{i}^k - \sum_{j \in \mathcal{C}_i} f_{i,j}^k = 0, &\forall i,k \IEEEeqnarraynumspace \label{Eq: P Balance SC} \\
    & (\psi^k_{i,j}){:} &  f_{i,j}^k - \frac{\tau^{l,k}_{i,j}}{X_{i,j}} \left(\theta_i^k - \theta_j^k\right) = 0,\quad &\forall i, j \in \mathcal{C}_i \\
    & (\eta^{+,k}_{i,j}){:} &  f_{i,j}^k \leq \overline{F}_{i,j}, &\forall i, j \in \mathcal{C}_i, k\IEEEeqnarraynumspace\\
    & (\eta^{-,k}_{i,j}){:} &  -f_{i,j}^k \leq -\overline{F}_{i,j}, &\forall i, j \in \mathcal{C}_i,k \IEEEeqnarraynumspace\label{Eq: Fmax}\\
    & (\chi^k_u){:} &  \sum_{i=1}^{n}\alpha_{i,u}^k = 1, & \forall u,k \IEEEeqnarraynumspace\label{Eq: Alpha1 SC}\\
    & (\gamma^k){:} &  \sum_{i=1}^{n}\alpha_{i}^k = 1, \label{Eq: }\\
    & (\kappa^k_i){:} &  \alpha_i^k \boldsymbol{\Omega}^k = \sum_u \left(\alpha_{i,u}^k\boldsymbol{\omega}_u^k\right), & \forall i,k \IEEEeqnarraynumspace\label{Eq: Alpha i kappa SC} \\ 
    & (\rho^{+,k}_i){:} &  p_{i}^k - p_{i}^{k=0}\leq r^\text{up}_{i}, &\forall i,k \ne 0 \IEEEeqnarraynumspace\label{Eq: PmaxI Res SC}\\
    & (\rho^{-,k}_i){:} &  p_{i}^{k=0}-p_{i}^k\leq r^\text{dw}_{i}, &\forall i,k \ne 0 \IEEEeqnarraynumspace\label{Eq: PminI Res SC}\\
    & (\delta^{+,k}_i){:} &  \mathbb{P}[\boldsymbol{p}_{i}^k\leq \tau^{g,k}_{i}\overline{P}_{i}]\geq 1-\epsilon_{g}, &\forall i,k \IEEEeqnarraynumspace\label{Eq: PmaxI SC}\\
    & (\delta^{-,k}_i){:} &  \mathbb{P}[-\boldsymbol{p}_{i}^k\leq -\tau^{g,k}_{i}\underline{P}_{i}]\geq 1-\epsilon_{g}, &\forall i,k. \IEEEeqnarraynumspace\label{Eq: PminI SC}
    \vspace{-4\jot}
\end{IEEEeqnarray}
\end{subequations}
\nomenclature[I]{$k \in \{0,...,\mathcal{K}\}$}{Contingency states \hfill}
\nomenclature[P]{$\tau^{l,k}_{i,j}$}{Binary parameter indicating whether the line ${i,j}$ is active during contingency $k$\hfill}
\nomenclature[P]{$\tau^{g,k}_{i}$}{Binary parameter indicating whether the generator $i$ is active during contingency $k$\hfill}
\nomenclature[P]{$\widetilde{\tau}^{k}_{u}$}{Binary parameter indicating whether the uncontrollable renewable generator $u$ is active during contingency $k$\hfill}
\end{model}

For the preventive security-constrained OPF, the generators scheduling must be equal for all contingency states: $p_i^{k=0} = p_i^k$.

The corrective security-constrained OPF is enforced by \eqref{Eq: PmaxI Res SC} and \eqref{Eq: PminI Res SC}.

\subsection{Pricing}
\subsubsection{Balancing prices}
In the security-constrained OPF with symmetric balancing, the calculation of the balancing prices is performed in the same as in Section \ref{Sec: Symmetric OPF}, but there will be a balancing price for each contingency: $\pi^{\alpha,k}, \pi^{\alpha,k}_{u}$. A price per contingency also applies for the asymmetric cases. 

\subsubsection{Reserve Prices} the upward and downward reserve prices are given by
\begin{IEEEeqnarray}{rCll}
    \pi^\text{up}_i &=& c^\text{up}_i-\sum_k \rho^{+,k}_i, \qquad &\forall i \IEEEyesnumber\IEEEyessubnumber*\IEEEeqnarraynumspace\\
    \pi^\text{dw}_i &=& c^\text{dw}_i-\sum_k \rho^{-,k}_i, \qquad &\forall i. \IEEEeqnarraynumspace
\end{IEEEeqnarray}
The upward and downward reserve prices, respectively $\pi^\text{up}_i$ and $\pi^\text{dw}_i$, depend on the reserve provision costs $c^\text{up}_i$ and $c^\text{dw}_i$, and on the dual multiplier of \eqref{Eq: PmaxI Res SC} and \eqref{Eq: PminI Res SC}. 

The dual multipliers $\rho^{+,k}_i$ and $\rho^{-,k}_i$ can only be greater than zero when the reserve capacity limits are enforced, i.e., when the contingency $k$ forces the generator $i$ to use of all of its reserve. When constraints \eqref{Eq: PmaxI Res SC} and \eqref{Eq: PminI Res SC} are non-binding, the dual multipliers are equal to zero.

Since the term $\sum_k \rho^{\text{+/-},k}_i$ is non-negative, the reserve prices decrease for generator $i$ when it is constrained in its reserve capacity provision. Thus, when constraints \eqref{Eq: PmaxI Res SC} and \eqref{Eq: PminI Res SC} are binding, generator $i$ incurs in marginally unprofitable operation, i.e, $ c^\text{up/dw}_i - \pi^\text{up/dw}_i > 0$.

It must be noted that reserve provision and pricing only applies for corrective security-constrained OPF, since in the preventive case reserves are equal to zero, i.e., pre-contingency and post-contingency scheduled generation are equal.

\subsubsection{Energy prices} the energy prices in the security-constrained case are given by

\begin{IEEEeqnarray}{C}
    \pi^\text{p,sc}_i = 2 c_{2,i} p_{i}+c_{1,i} {+} \delta_{i}^{+} {-} \delta_{i}^{-} {+} \sum_k \left[ \rho^{-,k}_i {-} \rho^{+,k}_i \right], \quad \forall i. \label{Eq: Eprice SC} \IEEEyesnumber\IEEEeqnarraynumspace
\end{IEEEeqnarray}

It can be seen that \eqref{Eq: Eprice SC} can be written in terms of the prices derived in Section \ref{Sec: Symmetric OPF} as:

\begin{IEEEeqnarray}{rCll}
    \pi^\text{p,sc}_i &=& \pi^\text{p}_i + \pi^\text{sc}_i , \quad &\forall i \label{Eq: Eprice SC 2} \IEEEyesnumber\IEEEeqnarraynumspace\\
    \noalign{\text{where}} \IEEEnonumber\\
    \pi^\text{sc}_i &=& \sum_k \left[ \rho^{-,k}_i - \rho^{+,k}_i \right], \quad & \forall i. \label{Eq: Pi SC} \IEEEyessubnumber*
\end{IEEEeqnarray}

Expression \eqref{Eq: Eprice SC 2} shows that the energy prices in the SC-OPF depend on the energy prices in the traditional OPF $\pi^\text{p}_i$ and a security price $\pi^\text{sc}_i$, as presented analytically by \textit{Arroyo and Galiana} \cite{Arroyo2005}. The security price increases for operations in which the downward reserves are activated to their full capacity, and decreases for the upward case.

As with reserves, expression \eqref{Eq: Pi SC} yields an intuitive price on the corrective case. General security prices can be rewritten in terms of the electricity prices and capacity limits at the different contingency cases by

\begin{IEEEeqnarray}{rCll}
    \pi^\text{sc}_i &=& \sum_k \left[ \delta^{+,k}_i - \delta^{-,k}_i - \lambda^{k}_i 
    \right], \quad & \forall i. \label{Eq: Pi SC} \IEEEyessubnumber*
\end{IEEEeqnarray}

Thus, the security prices increase when the generators are constrained by their maximum capacity on any of the contingency states, and decrease when the minimum capacity is binding. Security prices also increase by the marginal cost of generation during contingencies ($\lambda_i^k \le 0$).

